RegionDrag: Fast Region-Based Image Editing with Diffusion Models

Point-drag-based image editing methods, like DragDiffusion, have attracted significant attention. However, point-drag-based approaches suffer from computational overhead and misinterpretation of user intentions due to the sparsity of point-based editing instructions. In this paper, we propose a region-based copy-and-paste dragging method, RegionDrag, to overcome these limitations. RegionDrag allows users to express their editing instructions in the form of handle and target regions, enabling more precise control and alleviating ambiguity. In addition, region-based operations complete editing in one iteration and are much faster than point-drag-based methods. We also incorporate the attention-swapping technique for enhanced stability during editing. To validate our approach, we extend existing point-drag-based datasets with region-based dragging instructions. Experimental results demonstrate that RegionDrag outperforms existing point-drag-based approaches in terms of speed, accuracy, and alignment with user intentions. Remarkably, RegionDrag completes the edit on an image with a resolution of 512x512 in less than 2 seconds, which is more than 100x faster than DragDiffusion, while achieving better performance. Project page: https://visual-ai.github.io/regiondrag.

==> figure_tex/alpha.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.95\linewidth]{figure/alpha.pdf}
    \caption{Results of applying different noise weight \(\alpha\).}
    \label{fig:alpha}
\end{figure*}

==> figure_tex/mean_dist.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[height=4cm, keepaspectratio]{figure/mean_dist.pdf}
    \caption{Illustration of Mean Distance computation. Updated handle points are searched inside the search mask.}
    \label{fig:mean_distance}
\end{figure*}

==> figure_tex/results.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.9\linewidth]{figure/results.pdf}
    \caption{Quantitative analysis on various dragging methods. LPIPS ($\downarrow$) and Mean Distance ($\downarrow$) are reported. Results are produced on DragBench-S(R) and DragBench-D(R). The approach with better results should be located at the lower-left corner of the coordinate plane.}
    \label{fig:results}
\end{figure*}

==> table_tex/results.tex <==
\begin{table}[ht]
\centering
\caption{Ablation study}
\label{tab:results}
{\scriptsize % This will make the font smaller for the entire table content
\begin{tabular}{lcccc}
\toprule
Method & \multicolumn{2}{c}{DragBench-S(R)} & \multicolumn{2}{c}{DragBench-D(R)} \\
       & MD (\(\downarrow\)) & LPIPS (\(\downarrow\)) & MD (\(\downarrow\)) & LPIPS (\(\downarrow\)) \\
\midrule
SDEDrag\cite{nie2023blessing}             & 7.5           & 12.4             & 8.1           & 14.9             \\
DragDiffusion\cite{shi2023dragdiffusion}  &7.0             & 18.0             & \textbf{6.7}  & 11.5             \\
DiffEditor\cite{mou2024diffeditor}        & 23.6          & 17.6             & 22.1          & 10.9             \\
Ours                                      & \textbf{6.4}  & \textbf{8.9}     & 6.8           & \textbf{6.3}     \\
\midrule
Single-step copy paste & 6.5 & 9.6 & 11.1 & 6.3 \\
w/o mask color         & 6.4 & 9.8 &  \textbf{6.6} & 8.9 \\
Ours                   & \textbf{6.4} & \textbf{8.9} & 6.8 & \textbf{6.3} \\
\bottomrule
\end{tabular}
} % End of \footnotesize
\end{table}

